A Domain Specific Language for Testing Consensus Implementations

Large-scale, fault-tolerant, distributed systems are the backbone for many critical software services. Since they must execute correctly in a possibly adversarial environment with arbitrary communication delays and failures, the underlying algorithms are intricate. In particular, achieving consistency and data retention relies on intricate consensus (state machine replication) protocols. Ensuring the reliability of implementations of such protocols remains a significant challenge because of the enormous number of exceptional conditions that may arise in production. We propose a methodology and a tool called Netrix for testing such implementations that aims to exploit programmer's knowledge to improve coverage, enables robust bug reproduction, and can be used in regression testing across different versions of an implementation. As evaluation, we apply our tool to a popular proof of stake blockchain protocol, Tendermint, which relies on a Byzantine consensus algorithm, a benign consensus algorithm, Raft, and BFT-Smart. We were able to identify 4 deviations of the Tendermint implementation from the protocol specification and check their absence on an updated implementation. Additionally, we were able to reproduce 4 previously known bugs in Raft.

==> document/sections/implementation.tex <==
\section{{\toolname} Implementation}
\label{tool}

\textbf{\toolname} is written in the \texttt{go} programming language and is open source. \toolname exports \texttt{testlib} as a \texttt{go} library which developers can use to create and compose \texttt{TestCase} objects. The DSL primitives needed to describe filters are available as library functions. Two main components of \toolname are \texttt{APIServer} and \texttt{Dispatcher}. \texttt{APIServer} is used to receive events and messages from the replicas and \texttt{Dispatcher} is used to send messages to the replicas. All communication between \toolname and the replicas is achieved using the HTTP protocol. We plan to transition to protocol buffers to be able to automatically generate client libraries for other languages.

We instantiate the \texttt{APIServer, Dispatcher} components along with the \texttt{EventQueue} and \texttt{MessagePool} when the developer creates a \texttt{TestingServer}. \texttt{APIServer} runs a HTTP Server and implements the API interface for the replicas to communicate. The communication endpoints are,
\begin{enumerate}
  \item \textit{ReplicaEndpoint} - Receives Replica information and stores it in a dictionary indexed by the ReplicaID
  \item \textit{EventEndpoint} - Receives Events from the replicas and adds them to \texttt{EventQueue}.
  \item \textit{MessageEndpoint} - Receives Messages from the replicas and adds them to \texttt{MessagePool}
\end{enumerate}

\texttt{EventQueue} is dynamically allocated. \texttt{EventQueue.Subscribe} which returns a \texttt{go} channel. When Events are added, \texttt{EventQueue} pops an event from the head and publishes it to all the subscribers. We use the channel returned by \texttt{EventQueue.Subscribe} to drive the main test loop. Between successive unit tests, first we clear \texttt{EventQueue} and \texttt{MessagePool} and then send \texttt{Directive} messages instructing the replicas to restart.

For each unit tests, we record (1) the events received, (2) the messages received, and (3) the state transitions. We plan to introduce visualization tools to parse the log and better understand an unit test execution.

==> document/sections/instrumentation.tex <==
\section{Instrumentation}
\label{instrumentation}

An existing implementation of a consensus protocol needs to be modified such that \toolname receives all messages and events from the participating replicas. \toolname exposes an API to receives messages, events, and other necessary information from the replicas via RPC. We provide client libraries that developers can use to change their implementation's communication primitives. Figure~\ref{fig:instrumentation} illustrates the changes needed. Replicas first establish a connection to \toolname and communicate the relevant information. Earlier, replicas would communicate messages directly to each other. While testing with \toolname, for every message that a replica intends to send, the replica should first communicate an event of type message-send tagged with the message identifier and then submit the message to \toolname.

\toolname instructs the replicas to reset between successive unit tests to ensure the same start conditions for each test. \toolname uses special \texttt{Directive} messages to convey restart instructions. Other \texttt{Directive} messages instruct replicas to start or stop. Filter actions can issue directives to the replicas. Developers should change the implementation to accept \texttt{Directive} messages and perform the requested action. To aid the developer with the changes, we provide client libraries. Each replica runs an instance of the library and uses it to communicate to \toolname. The libraries are currently available in \texttt{go} language with development planned for other languages. The library interface is as follows,
\begin{enumerate}
  \item \textbf{Init} - accepts information needed to communicate \toolname and establishes the connection.
  \item \textbf{SendMessage} - accepts messages as a sequence of bytes along with the recipients identification. Internally, it communicates a message-send event and the message to \toolname.
  \item \textbf{ReceiveMessage} - returns any messages that are communicated to the current replica by \toolname. Internally, it communicates a message-receive event to \toolname before returning the contents of the message.
  \item \textbf{SendEvent} - accept event type and other parameters and can be used to communicate other events.
\end{enumerate}

\noindent Replicas communicate messages as a sequence of bytes. Therefore, the developer has to plug in the serialization and de-serialization adapter when writing the tests. \toolname de-serializes the messages received using the adapter. Some filter conditions are specified based on the contents of the de-serialized messages.

